The Topological BERT: Transforming Attention into Topology for Natural Language Processing

In recent years, the introduction of the Transformer models sparked a revolution in natural language processing (NLP). BERT was one of the first text encoders using only the attention mechanism without any recurrent parts to achieve state-of-the-art results on many NLP tasks. This paper introduces a text classifier using topological data analysis. We use BERT's attention maps transformed into attention graphs as the only input to that classifier. The model can solve tasks such as distinguishing spam from ham messages, recognizing whether a sentence is grammatically correct, or evaluating a movie review as negative or positive. It performs comparably to the BERT baseline and outperforms it on some tasks. Additionally, we propose a new method to reduce the number of BERT's attention heads considered by the topological classifier, which allows us to prune the number of heads from 144 down to as few as ten with no reduction in performance. Our work also shows that the topological model displays higher robustness against adversarial attacks than the original BERT model, which is maintained during the pruning process. To the best of our knowledge, this work is the first to confront topological-based models with adversarial attacks in the context of NLP.

==> background.tex <==
\section{BERT Model}
\input{bert}

\section{Attention Maps and Attention Graphs}
\input{attention_maps_and_graphs}

\section{Persistent Homology}\label{sec:persistent_homology}
\input{persistent_homology}

\section{Persistence Images}
\input{persistence_image}

==> gradcam_study.tex <==
Instead of exploring the structure of the persistence diagrams, we investigate what part of the input is most relevant for the model to predict the class of the sentence. 
To do so, we develop a method inspired by GradCam (\cite{gradcam}). 

GradCam is used to help understand the decisions made by deep learning models. 
Given an image, GradCam produces a heatmap that shows how the model makes its decision for that image. 
In our case, as the input is composed of either 288 (twice the number of heads) or 432 images (three times the number of heads), we can not directly apply the method proposed by \cite{gradcam}. 
Instead, we compute the gradient of the output logit with respect to the input image. 
This yields a tensor of the same shape as the input (for example for the ordinary case, the shape is [288, 50, 5]). 
Then we average the absolute value of the gradient over each channel to obtain a number that represents the influence of each individual image on the model output. 
Finally, we take the mean of these values corresponding to images coming from the same attention head (two images in the case of the ordinary filtration, three for the others). 
We end up with a score for the 144 heads of BERT for one input sentence. 
We perform this procedure for a large number of sentences and average all the obtained scores. 

Our hypothesis is that the higher the score of a head, the more relevant it is to the topological model, and the more information about the sentence structure with respect to the current task it contains. 
\cref{fig:best_heads_scores} displays the 30 best attention heads of the topological model trained on the PI-dataset \enquote{CoLA, 4 Epochs, Ordinary}, but with various numbers of sentences considered and for different symmetry functions.

\begin{figure}[H]
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_max_50_sent_30_best.png}
      \caption{max and 50 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_max_50_sent}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_max_500_sent_30_best.png}
      \caption{max and 500 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_max_500_sent}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_max_5000_sent_30_best.png}
      \caption{max and 5000 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_max_5000_sent}
    \end{subfigure}

    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_min_50_sent_30_best.png}
      \caption{min and 50 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_min_50_sent}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_min_500_sent_30_best.png}
      \caption{min and 500 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_min_500_sent}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_min_5000_sent_30_best.png}
      \caption{min and 5000 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_min_5000_sent}
    \end{subfigure}

    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_mean_50_sent_30_best.png}
      \caption{mean and 50 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_mean_50_sent}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_mean_500_sent_30_best.png}
      \caption{mean and 500 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_mean_500_sent}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.3\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/cola_model_4_ordinary_mean_5000_sent_30_best.png}
      \caption{mean and 5000 sentences}
      \label{fig:30_best_heads_cola_model_4_ordinary_mean_5000_sent}
    \end{subfigure}

    \caption{Scores of the 30 best heads for variations of models over the PI-dataset \enquote{CoLA, 4 Epochs, Ordinary, max}. The x-axis is the head id and the y-axis is the layer id.}
    \label{fig:best_heads_scores}
\end{figure}

The heads with the highest scores are independent of the number of sentences used, as there is almost no difference in \cref{fig:30_best_heads_cola_model_4_ordinary_max_50_sent,fig:30_best_heads_cola_model_4_ordinary_max_500_sent,fig:30_best_heads_cola_model_4_ordinary_max_5000_sent}, \cref{fig:30_best_heads_cola_model_4_ordinary_min_50_sent,fig:30_best_heads_cola_model_4_ordinary_min_500_sent,fig:30_best_heads_cola_model_4_ordinary_min_5000_sent}, and \cref{fig:30_best_heads_cola_model_4_ordinary_mean_50_sent,fig:30_best_heads_cola_model_4_ordinary_mean_500_sent,fig:30_best_heads_cola_model_4_ordinary_mean_5000_sent}.
We also observed that the best performing heads are almost independent of the symmetry function considered.
In general, the best heads are located in the deep layers of BERT. 
Therefore, the heads of BERT located in the later layers are the ones that change the most when fine-tuning (\cite{dark_secret_of_bert}), and they are also the most relevant for the topological classifier.

We design the following experiment to determine if these high-scoring heads contain most of the necessary information for our topological classifier to perform well.
First we determine the head with the highest scores. 
We train a model on a selected PI-dataset $\alpha$ and we apply our rating procedure on it. 
We look at the $n$ heads with the highest score (for $n$ = 70, 50, 30, 10, 5, 3, 2, and finally the best head).
Then, we train another model on a PI-dataset $\beta$ but with persistence images only related to the $n$ highest scoring heads.
When considering the 70 best heads, we do not consider the persistence images from the other 74 for heads. 
In the case of the Ordinary filtration the input of shape [288, 50, 5] is pruned to the shape [140, 50, 5], as each head produces two persistence images (one for the 0-dimensional features, one for the 1-dimensional features). 
\cref{Tab:table_best_heads_results_base} presents the performance obtained from such a pruning. 
The base PI-dataset considered is \enquote{CoLA, 4 Epochs, Ordinary, max}.
The other columns are variations of the base PI-dataset by changing either the considered symmetry function or the number of fine-tuning epochs. 
In \cref{Tab:table_best_heads_results_base} the PI-dataset $\alpha$ is the base PI-dataset and the PI-dataset $\beta$ is the PI-dataset identified by the column.
In \cref{Tab:table_best_heads_results_base_specific}, $\alpha$ and $\beta$ are both the PI-dataset identified by the column. 

\begin{table}[H]
    \centering
    \begin{tabularx}{1.0\textwidth} { |
            >{\raggedright\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X |}
         \hline
         \hline
          & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Min}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Mean}} & \textbf{\thead{CoLA \\ 10 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 20 Epochs \\ Ordinary \\ Max}}\\
          \hline
          \textbf{BERT} & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.561~/~82.2$ & $\mathbf{0.591~/~83.3}$\\
          \hline
          144 Heads & $0.539~/~81.2$ & $\underline{0.548~/~81.5}$ & $0.546~/~81.2$ & $0.585~/~83.0$ & $\mathbf{0.591~/~83.3}$\\
          70 Heads & $0.557~/~81.3$ & $\mathbf{0.552~/~81.7}$ & $0.544~/~80.6$ & $0.581~/~82.9$ & $0.587~/~83.2$\\   
          50 Heads & $0.557~/~81.2$ & $0.545~/~81.5$ & $0.551~/~81.2$ & $0.580~/~82.7$ & $\underline{0.590~/~83.3}$\\   
          30 Heads & $\mathbf{0.582~/~82.4}$ & $\underline{0.548~/~81.5}$ & $0.548~/~80.9$ & $0.584~/~83.0$ & $0.578~/~82.8$\\
          10 Heads & $0.545~/~81.0$ & $0.540~/~81.2$ & $0.555~/~81.6$ & $0.589~/~83.1$ & $0.574~/~82.5$\\
          5 Heads & $0.553~/~81.7$ & $0.519~/~80.6$ & $\mathbf{0.563~/~81.9}$ & $\underline{0.594~/~83.3}$ & $0.590~/~83.2$\\
          3 Heads & $0.554~/~81.9$ & $0.504~/~80.0$ & $\underline{0.556~/~81.6}$ & $\mathbf{0.594~/~83.4}$ & $0.583~/~82.9$\\
          2 Heads & $\underline{0.560~/~82.1}$ & $0.497~/~79.8$ & $0.525~/~80.3$ & $0.582~/~82.9$ & $0.582~/~82.9$\\
          1 Head & $0.492~/~79.4$ & $0.469~/~78.7$ & $0.479~/~78.7$ & $0.459~/~77.4$ & $0.535~/~80.7$\\
          \hline
          \hline
    \end{tabularx}
    \caption{Performances of the topological models while considering different number of high scoring heads. \textbf{These are determined from the base PI-dataset \enquote{CoLA, 4 Epochs, ordinary, max}.}}
    \label{Tab:table_best_heads_results_base}
\end{table}

\begin{table}[H]
    \centering
    \begin{tabularx}{1.0\textwidth} { |
            >{\raggedright\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X |}
         \hline
         \hline
          & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Min}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Mean}} & \textbf{\thead{CoLA \\ 10 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 20 Epochs \\ Ordinary \\ Max}}\\
          \hline
          \textbf{BERT} & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.561~/~82.2$ & $0.591~/~83.3$\\
          \hline
          144 Heads & $0.539~/~81.2$ & $\underline{0.548~/~81.5}$ & $0.546~/~81.2$ & $0.585~/~83.0$ & $0.591~/~83.3$\\
          70 Heads & $0.557~/~81.3$ & $0.539~/~81.0$ & $0.553~/~81.6$ & $0.571~/~82.6$ & $\mathbf{0.601~/~83.7}$\\   
          50 Heads & $0.557~/~81.2$ & $\mathbf{0.557~/~81.9}$ & $0.556~/~81.7$ & $0.582~/~82.9$ & $0.591~/~83.3$\\   
          30 Heads & $\mathbf{0.582~/~82.4}$ & $0.541~/~81.4$ & $0.537~/~81.2$ & $0.576~/~82.6$ & $0.581~/~82.9$\\
          10 Heads & $0.545~/~81.0$ & $0.547~/~81.4$ & $\underline{0.556~/~81.8}$ & $\underline{0.592~/~83.1}$ & $\underline{0.581~/~83.4}$\\
          5 Heads & $0.553~/~81.7$ & $0.518~/~80.5$ & $0.555~/~81.6$ & $0.587~/~83.0$ & $0.591~/~83.3$\\
          3 Heads & $0.554~/~81.9$ & $0.500~/~79.9$ & $\mathbf{0.569~/~82.1}$ & $\mathbf{0.590~/~83.2}$ & $0.579~/~82.7$\\
          2 Heads & $\underline{0.560~/~82.1}$ & $0.500~/~80.0$ & $0.527~/~80.4$ & $0.578~/~82.7$ & $0.579~/~82.7$\\
          1 Head & $0.492~/~79.4$ & $0.463~/~78.5$ & $0.487~/~79.0$ & $0.458~/~77.8$ & $0.539~/~80.9$\\
          \hline
          \hline
    \end{tabularx}
    \caption{Performances of the topological models while considering different numbers of high scoring heads. \textbf{These are determined specifically for each PI-dataset.}}
    \label{Tab:table_best_heads_results_base_specific}
\end{table}

The performance of the topological classifier trained on the base PI-dataset does not decrease with decreasing number of input images. 
It is even increasing and outperforms the 144 heads model at most by 2\% in accuracy on the prediction set. 
Astonishingly, with 2 heads, our topological classifier outperforms BERT by 1.5\% in accuracy. 
The model receives only 4 images of the initial 288, and its accuracy is still very large. 
It diminishes when considering only one head, but it still has a high accuracy of almost 80\%.

The same trend can be observed for all the other PI-datasets: an increasing or constant accuracy when we decrease the number of considered heads from 70 to 10. However, we get a lower accuracy when we only consider less than ten heads.
In all the models, decreasing the number of input images increases the performance of our topological classifier, up to a certain minimal number of heads considered. 
Choosing a model-specific rating of heads does not change the behavior in the results, neither in the trend nor in values. 
Hence the heads containing the most relevant information with respect to our topological classifier are consistent across different symmetry functions and number of fine-tuning epochs.

We do not observe the same phenomenon when we look at different datasets. 
\cref{Tab:table_best_heads_results_tasks,,Tab:table_best_heads_results_tasks_specific} display the performance of the topological classifiers applied to the different datasets. 
In \cref{Tab:table_best_heads_results_tasks}, the best scoring heads come from a model trained on the base PI-dataset, and the evaluated model hyperparameters are optimized on the CoLA dataset. 
In \cref{Tab:table_best_heads_results_tasks_specific}, the best scoring heads come from a model trained on the PI-dataset mentioned in the column, and the evaluated model is specific to the current dataset. 

\begin{table}[H]
    \centering
    \begin{tabularx}{1.0\textwidth} { |
            >{\raggedright\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X |}
         \hline
         \hline
          & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{IMDB \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{SPAM \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{SST2 \\ 4 Epochs \\ Ordinary \\ Max}} \\
          \hline
          \textbf{BERT} & $0.518~/~80.6$ & $\mathbf{0.843~/~92.2}$ & $\underline{0.993~/~99.8}$ & $\mathbf{0.853~/~92.7}$ \\
          \hline
          144 Heads & $0.539~/~81.2$ & $\underline{0.776~/~88.8}$ & $\mathbf{0.999~/~99.9}$ & $\underline{0.799~/~89.8}$ \\
          70 Heads & $0.557~/~81.3$ & $0.664~/~83.0$ & $\underline{0.993~/~99.8}$ & $0.784~/~89.2$ \\   
          50 Heads & $0.557~/~81.2$ & $0.611~/~79.1$ & $0.957~/~98.9$ & $0.782~/~89.1$ \\   
          30 Heads & $\mathbf{0.582~/~82.4}$ & $0.596~/~79.1$ & $\underline{0.993~/~99.8}$ & $0.771~/~88.5$ \\
          10 Heads & $0.545~/~81.0$ & $0.413~/~70.7$ & $0.993~/~99.5$ & $0.766~/~88.3$ \\
          5 Heads & $0.553~/~81.7$ & $0.412~/~70.1$ & $0.978~/~99.5$ & $0.459~/~72.4$ \\
          3 Heads & $0.554~/~81.9$ & $0.395~/~65.4$ & $0.948~/~98.6$ & $0.460~/~72.7$ \\
          2 Heads & $\underline{0.560~/~82.1}$ & $0.231~/~60.6$ & $0.710~/~93.6$ & $0.307~/~63.5$ \\
          1 Head & $0.492~/~79.4$ & $0.184~/~57.4$ & $0.396~/~88.0$ & $-0.026~/~48.6$ \\
          \hline
          \hline
    \end{tabularx}
    \caption{Performances of the topological models from the different tasks while considering different amounts of high scoring heads. These are determined from the base PI-dataset, and \textbf{the evaluated model is specific to CoLA.}}
    \label{Tab:table_best_heads_results_tasks}
\end{table}

\begin{table}[H]
    \centering
    \begin{tabularx}{1.0\textwidth} { |
            >{\raggedright\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X |}
         \hline
         \hline
          & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{IMDB \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{SPAM \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{SST2 \\ 4 Epochs \\ Ordinary \\ Max}} \\
          \hline
          \textbf{BERT} & $0.518~/~80.6$ & $\mathbf{0.843~/~92.2}$ & $0.993~/~99.8$ & $\mathbf{0.853~/~92.7}$ \\
          \hline
          144 Heads & $0.539~/~81.2$ & $\underline{0.787~/~89.4}$ & $\underline{0.999~/~99.9}$ & $0.799~/~89.8$ \\
          70 Heads & $0.557~/~81.3$ & $0.777~/~89.0$ & $0.993~/~99.8$ & $0.780~/~89.0$ \\   
          50 Heads & $0.557~/~81.2$ & $0.762~/~88.2$ & $0.993~/~99.8$ & $0.767~/~88.3$ \\   
          30 Heads & $\mathbf{0.582~/~82.4}$ & $0.783~/~89.3$ & $\mathbf{1.0~/~100}$ & $\underline{0.798~/~89.9}$ \\
          10 Heads & $0.545~/~81.0$ & $0.779~/~89.0$ & $0.993~/~99.8$ & $0.778~/~88.9$ \\
          5 Heads & $0.553~/~81.7$ & $0.770~/~88.6$ & $0.836~/~95.5$ & $0.789~/~89.5$ \\
          3 Heads & $0.554~/~81.9$ & $0.767~/~88.5$ & $0.831~/~95.5$ & $0.745~/~87.3$ \\
          2 Heads & $\underline{0.560~/~82.1}$ & $0.695~/~84.8$ & $0.786~/~94.4$ & $0.717~/~85.8$ \\
          1 Head & $0.492~/~79.4$ & $0.560~/~77.2$ & $0.772~/~94.3$ & $0.721~/~85.9$ \\
          \hline
          \hline
    \end{tabularx}
    \caption{Performances of the topological models from the different tasks while considering different amounts of high scoring heads. These are determined for each PI-datasets, and \textbf{the evaluated model is specific to the current task.}}
    \label{Tab:table_best_heads_results_tasks_specific}
\end{table}

For the head scores from CoLA, the performance of the model on the other tasks decreases with decreasing number of considered images. 
But when the head scores are determined for each PI-dataset, the performance remains constant when at least 10 heads are considered, and decreases slowly when less than 10 heads are considered. 
For the SPAM dataset, we even observe a perfect score of 100\% accuracy obtained while considering 30 heads.
The boosting effect of pruning images are the most significant for the CoLA dataset. 

We also consider the effect of image pruning for other filtrations: \cref{tab:table_best_heads_results_filtrations} presents the result for the CoLA dataset, but considering various types of persistent homology. The head scoring is determined for each PI-dataset.

\begin{table}[H]
    \centering
    \begin{tabularx}{1.0\textwidth} { |
            >{\raggedright\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X |}
         \hline
         \hline
          & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 4 Epochs \\ MultiDim \\ Max}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Directed \\ Max}} \\
          \hline
          \textbf{BERT} & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.518~/~80.6$ \\
          \hline
          144 Heads & $0.539~/~81.2$ & $0.552~/~81.5$ & $0.532~/~80.7$ \\
          70 Heads & $0.557~/~81.3$ & $0.544~/~81.2$ & $\mathbf{0.551~/~81.8}$ \\   
          50 Heads & $0.557~/~81.2$ & $0.546~/~81.1$ & $0.547~/~81.6$ \\   
          30 Heads & $\mathbf{0.582~/~82.4}$ & $\mathbf{0.561~/~82.0}$ & $\underline{0.548~/~81.6}$ \\
          10 Heads & $0.545~/~81.0$ & $0.555~/~81.5$ & $0.538~/~81.2$ \\
          5 Heads & $0.553~/~81.7$ & $0.557~/~81.6$ & $0.528~/~80.9$ \\
          3 Heads & $0.554~/~81.9$ & $0.554~/~81.6$ & $0.538~/~81.0$ \\
          2 Heads & $\underline{0.560~/~82.1}$ & $\underline{0.556~/~81.7}$ & $0.503~/~79.7$ \\
          1 Head & $0.492~/~79.4$ & $0.485~/~79.2$ & $0.455~/~78.1$ \\
          \hline
          \hline
    \end{tabularx}
    \caption{Performances of the topological models for different types of persistent homology for the CoLA dataset while considering different amounts of high scoring heads. These are determined specifically for each PI-dataset.}
    \label{tab:table_best_heads_results_filtrations}
\end{table}

Again, pruning the images is beneficial for performance, with a more significant effect for the Ordinary and Directed filtrations. 
Without pruning, the MultiDim filtration outperforms the others, but the ordinary persistence combined with pruning reaches the same peak performance of 82\% in accuracy. 
Interestingly, to increase the performance of the topological classifier, one should prefer to remove some well-chosen input images, rather than considering more complex and computation-demanding filtrations. 

The highest-rated heads may not be the only ones from which the model retrieves valuable information. 
To explore this, we trained the model while keeping the images coming from all the attention heads except the heads with the highest rating. 
\cref{Tab:table_best_heads_results_inverted} shows the result for different symmetry functions and a different number of fine-tuning epochs. 
Here, the line \textit{10 heads} corresponds to the performance obtained by the model while trained on images from 134 attention heads (we removed the images from the 10 best heads). 


\begin{table}[H]
    \centering
    \begin{tabularx}{1.0\textwidth} { |
            >{\raggedright\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X :
            >{\raggedleft\arraybackslash}X |}
         \hline
         \hline
          & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Min}} & \textbf{\thead{CoLA \\ 4 Epochs \\ Ordinary \\ Mean}} & \textbf{\thead{CoLA \\ 10 Epochs \\ Ordinary \\ Max}} & \textbf{\thead{CoLA \\ 20 Epochs \\ Ordinary \\ Max}}\\
          \hline
          \textbf{BERT} & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.518~/~80.6$ & $0.561~/~82.2$ & $0.591~/~83.3$\\
          \hline
          70 Heads & $0.0~/~30.9$ & $0.540~/~81.2$ & $0.0~/~30.9$ & $0.562~/~81.9$ & $0.0~/~30.9$\\   
          50 Heads & $0.486~/~79.4$ & $0.505~/~80.1$ & $0.492~/~15.9$ & $0.564~/~82.2$ & $\underline{0.593~/~83.4}$\\   
          30 Heads & $0.517~/~80.4$ & $\mathbf{0.559~/~82.0}$ & $0.499~/~79.6$ & $0.565~/~82.4$ & $0.573~/~82.7$\\
          10 Heads & $0.533~/~80.9$ & $\underline{0.538~/~81.3}$ & $0.484~/~76.6$ & $0.574~/~82.7$ & $0.584~/~83.0$\\
          5 Heads & $0.514~/~80.4$ & $0.536~/~81.2$ & $\mathbf{0.545~/~81.6}$ & $0.561~/~82.0$ & $0.583~/~83.0$\\
          3 Heads & $\underline{0.537~/~80.9}$ & $0.531~/~81.1$ & $\underline{0.531~/~81.1}$ & $\underline{0.574~/~82.7}$ & $0.573~/~82.6$\\
          2 Heads & $0.540~/~80.7$ & $0.546~/~80.9$ & $0.526~/~80.9$ & $0.585~/~82.5$ & $\mathbf{0.593~/~83.4}$\\
          1 Head & $\mathbf{0.537~/~81.0}$ & $0.525~/~80.8$ & $0.538~/~80.3$ & $\mathbf{0.584~/~82.7}$ & $0.566~/~82.4$\\
          \hline
          \hline
    \end{tabularx}
    \caption{Performances of the topological models while removing different numbers of high scoring heads. For examples, \textit{5 heads} means that we removed the images generated by the 5 best heads, always determined from the base model.}
    \label{Tab:table_best_heads_results_inverted}
\end{table}

The general tendency is a constant performance while the number of considered images increases. 
The exceptions are for the \textit{mean} symmetry function where a neat increase in accuracy occurs, and the low accuracy when only half of the worst performing heads are considered. 

These results verify the statements proposed by \cite{bert_plays_lottery} that one can find a good sub-model inside BERT even when it is highly pruned. 
In \cite{are_sixteen_heads_better_than_one}, some layers where pruned to one head with no effect on performance. 
With our procedure, we could reduce the number of head to five without a loss of performance.

From all these experiments, a clear observation arises: specific heads are highly relevant for our model to perform comparably to BERT or even outperform it. 
To investigate what these heads look like, we plot the attention maps (\cite{dark_secret_of_bert}) for the three best heads of our base PI-dataset (\enquote{CoLA, 4 Epochs, Ordinary, max}) for ten sentences in class 1 (grammatically correct) and 10 sentences in class 0 (grammatically incorrect). 

\begin{figure}[H]
    \begin{subfigure}{.95\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/attention_map_best_3_heads_class_1.png}
      \caption{Attention maps corresponding to sentences in class 1.}
      \label{fig:attention_maps_best_3_heads_class_1}
    \end{subfigure}

    \begin{subfigure}{.95\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{pictures/attention_map_best_3_heads_class_0.png}
      \caption{Attention maps corresponding to sentences in class 0.}
      \label{fig:attention_maps_best_3_heads_class_0}
    \end{subfigure}

    \caption{Attention maps of the 3 best heads of the PI-dataset \enquote{CoLA, 4 Epochs, Ordinary, max}. Each line corresponds to a head, the best one at the top. Sentences are part of the CoLA dataset.}
    \label{fig:attention_maps_best_3_heads}
\end{figure}

Almost all the feature maps have high values on the column corresponding to the [SEP] token. 
This means that to encode the sentence, the head will mainly consider the current vectorization of [SEP] to compute the new representation of each token. 
This suggests that this pattern contains sufficient information to get a good performance from the topological classifier. 
In \cite{what_does_bert_look_at}, this peculiar pattern on [SEP] is interpreted as a \textit{no-op} function; the default mode a head enters if it cannot apply its specific function. 
For example in (\cite{what_does_bert_look_at}) the authors found a head that is specialized in  verb-subject recognition. This head puts all the attention on [SEP] if the input word is not a verb. 
Our observation suggests that giving attention to [SEP] contains useful information, and is not only a way for the head to do no operation. 

To deduce how full attention on [SEP] can be used to classify sentences, the persistence images are of great help. 
\cref{fig:persistence_images_best_3_heads} plots the persistence images corresponding to the above attention maps.

\begin{figure}[H]
    \centering
    \includegraphics[width=.95\linewidth]{pictures/persistence_images_best_3_heads_both_class.png}
    \caption{Persistence images of the 3 best heads from the PI-dataset \enquote{CoLA, 4 Epochs, Ordinary, max}. 
    Each line corresponds to a head, the best one at the top. 
    The first 10 pictures refers to sentences in class 0, the last ten to class 1. 
    The persistence images represent the zero dimensional persistence features.}
    \label{fig:persistence_images_best_3_heads}
\end{figure}

These images correspond to attention almost exclusively on the token [SEP].
Each bar in the persistence image represents the filtration value where a token is connected to the [SEP] vertex. 
Sparse diagrams represent a filtration where the vertices are connected to the [SEP] vertex at different filtration values. Pack diagrams indicate a filtration where the vertices are connected to [SEP] in a narrow range of filtration values. 
The valuable information of the full-attention-to-[SEP] pattern might be in the connection to the [SEP] vertex in the attention graph, which is easily obtained by the topological classifiers.

But where does the model look when it processes persistence images? 
The regions that are the most relevant to the model appear when the gradient is visualized, as in \cref{fig:gradient_values_best_3_heads}.
The darker the red, the more the area influences the model towards class 0; the darker the blue, the more the influence is towards class 1. 
The white areas are not considered by the model as being relevant to the output classification.. 

\begin{figure}[H]
    \centering
    \includegraphics[width=.95\linewidth]{pictures/gradient_values_best_3_heads_both_class.png}
    \caption{Gradient values of each pixel from the PI-dataset \enquote{CoLA, 4 Epochs, Ordinary, max}.
    Each line corresponds to one head, and the lines are sorted by average importance score. 
    The first 10 pictures refers to sentences in class 0, the last ten to class 1. 
    The darker the red, the more the area influences the model towards class 0; the darker the blue, the more the influence is towards class 1. 
    The persistence images represent the zero dimensional persistence features.}
    \label{fig:gradient_values_best_3_heads}
\end{figure}

The model has different behavior for each sentence label. 
If the sentence is in class 0, any positive pixel value will decrease the model output, thus increasing the probability of class 0. 
This is independent of the death time of the feature, and hence only the existence is relevant. 
If the sentence belongs to class 1, then again, any point in the image will influence the output probability towards class 1, except for some particular regions generally situated at filtration values between $0.7$ and $0.8$, where the influence is inverted. 
Persistence features of dimension 0 that die at this filtration value influence the model output toward class 0. 
A 0-dimensional feature dies when it gets connected to the main connected component; hence if a vertex has edges with the lowest value in this specific filtration range, it will influence the model toward class 0. 

From the CoLA dataset perspective, a sentence containing such a token has a higher chance of being predicted as grammatically incorrect.



==> methodology_sections.tex <==
\section{Data}
\input{data_set_description}

\section{Model}
\label{sec}
\input{model_description}

\section{Hardware}
\input{hardware_description}

==> model_description.tex <==
We run the experiments on the \enquote{bert-base-uncased} model from the HuggingFace library (\cite{huggingface_transformers}) for the BERT baselines. 
We fine-tuned it for 4, 10, and 20 epochs \footnote{We follow the procedure proposed in \href{https://github.com/MohamedAteya/BERT-Fine-Tuning-Sentence-Classification-for-CoLA}{https://github.com/MohamedAteya/BERT-Fine-Tuning-Sentence-Classification-for-CoLA}} 
to study the importance of fine-tuning BERT with respect to the performance of the topological classifiers.
This gives use three BERT models per task, and each is used to transform sentences into persistence images. 

The choice of the symmetry function is a crucial step to get from the attention matrices to the non-directed attention graphs. 
To explore its relevance with respect to the performance of the topological classifier, we use four different symmetry functions: maximum, minimum, multiplication and mean.

We also consider the three types of filtrations describe in \cref{sec:persistent_homology}. 
Unfortunately, we are limited in terms of computation time and power as it can reach excessively high values depending on the length of the sentence to transform (see \cref{fig:image_computation_time}). 
Hence for the MultiDim filtration, we consider only the maximum as a symmetry function, and the Directed filtration is only applied to the CoLA dataset.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.7]{pictures/image_computation_time_plot.png}
    \caption{The computation time of the persistence images from the attention maps as a function of the number of tokens in a sequence for the three types of filtrations. Because of the high memory usage for the Directed version, we only plotted sequence lengths of a size up to 80 tokens for it.}
    \label{fig:image_computation_time}
\end{figure}

In total, one fine-tuned BERT model generates 5 or 6 persistence image datasets (PI-datasets). 
We refer to a PI-dataset by the fine-tuned BERT model producing it (name of the dataset and number of fine-tuning epochs), the type of filtration, and the symmetry function, e.g., \enquote{IMDB, 10 epochs, MultiDim, max}. 

Our topological classifiers are convolutional neural networks taking as input the stack of persistence images from one sentence. 
The architecture identified by running a hyperparameter search using the Optuna library (\cite{optuna}) for 500 trials tuning the number of convolution and fully connected layers, the learning rate, the optimizer, and the dropout rate. 
The hyperparameter search is done on one dataset (CoLA, IMDB, SPAM, or SST2), and we say that the model designed from the hyperparameter search result is specific to this dataset. 
We run hyperparameter searches for each classification task and type of filtration. 
The architectures of all the topological classifiers are presented in \cref{tab:architecture_of_topological_models}.

We then investigate the performance of a topological classifier specific to one dataset when evaluated on the other datasets.
To do so, for each PI-dataset, we evaluate the performance of two topological models: 
one whose hyperparameters are optimized on the current dataset, the other one specific to the CoLA dataset. 
We refer to the first model as the specific model and to the second as the general model. 

The inference time of our combination of the BERT model and the topological classifier is greater than the inference time of the BERT model itself.
When using the Ordinary filtration, the time needed to transform a tokenized sentence into a persistence image and predict its class is two times greater than the BERT prediction time.  
It goes up to 20 times for the MultiDim filtration and 70 times for the Directed filtration. The bottleneck is the computation of the persistence images from the persistence diagrams, which is not implemented on GPU but only on CPU.


